Image-Coupled Volume Propagation for Stereo Matching

Several leading methods on public benchmarks for depth-from-stereo rely on memory-demanding 4D cost volumes and computationally intensive 3D convolutions for feature matching. We suggest a new way to process the 4D cost volume where we merge two different concepts in one deeply integrated framework to achieve a symbiotic relationship. A feature matching part is responsible for identifying matching pixels pairs along the baseline while a concurrent image volume part is inspired by depth-from-mono CNNs. However, instead of predicting depth directly from image features, it provides additional context to resolve ambiguities during pixel matching. More technically, the processing of the 4D cost volume is separated into a 2D propagation and a 3D propagation part. Starting from feature maps of the left image, the 2D propagation assists the 3D propagation part of the cost volume at different layers by adding visual features to the geometric context. By combining both parts, we can safely reduce the scale of 3D convolution layers in the matching part without sacrificing accuracy. Experiments demonstrate that our end-to-end trained CNN is ranked 2nd on KITTI2012 and ETH3D benchmarks while being significantly faster than the 1st-ranked method. Furthermore, we notice that the coupling of image and matching-volume improves fine-scale details as demonstrated by our qualitative analysis.

==> 01_introduction.tex <==
moved to main


==> _03_backup.tex <==
\section{Methods}
\label{sec:methods}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{Overview}
The proposed model has four steps: feature extraction, cost volume construction, cost aggregation, and disparity regression.
Given a pair of left and right images $\mathbf{I}_l, \mathbf{I}_l \in \mathbb{R} ^ {3 \times H \times W}$, the feature extractor, a UNet-like CNNs\cite{ronneberger2015u}, produces the feature maps $\mathrm{f}_l, \mathrm{f}_r \in \mathbb{R}^{c_f \times h_0 \times w_0}$ where $h_0 = \left \lfloor H / 3 \right \rfloor$ and $w_0 = \left \lfloor W / 3 \right \rfloor$. The feature extractor begins with three layers of $3\times3$ 2D convolutions with output channels of 16, 32, and 32 and strides of 1, 3, and 1 to scale down the images at the third resolution, followed by a 3-level UNet.
Since the initial cost volume is constructed by group-wise correlation\cite{guo2019group} that requires a high dimension of feature maps, we use an asymmetric encoder-decoder structure to increase the output channels of the feature extractor.
The numbers of channels are 32, 64, and 128 for each level of encoder layers and 128 for all decoder layers by keeping the numbers subtracted by the feature number from the skip connection at the deconvolution layers, $\eg$ the last deconvolution convolves 128-channels into 96-channels to concatenate 32-channels skip connection.

To operate group-wise correlation, each feature map $\mathrm{f} \in \mathbb{R}^{c_f \times h_0 \times w_0}$ is split along the channel dimension into $c_0$ number of feature maps $\left\{ \mathrm{f}^{1}, \mathrm{f}^{2}, ..., \mathrm{f}^{c_0}\right\}$ where each $\mathrm{f}^{g}$ has $c_f/c_0$ number of channels. 
Each value in the initial cost volume $\mathbf{v}_0 \in \mathbb{R} ^ {c_0 \times d_0 \times h_0 \times w_0}$ is determined as 
\begin{align}
    \mathbf{v}_0\left(g, d, i, j\right)=\frac{1}{c_f / c_0}\left\langle\mathrm{f}_l^g(i, j), \mathrm{f}_r^g(i, j-d)\right\rangle
\end{align}
where $d_0 = \left \lfloor D / 3 \right \rfloor$ and $D$ is the maximum disparity.

The cost aggregation module has two parallel paths of UNet structures to evolve another left feature map $\mathbf{f}_{0}$ as well as the 3D cost volume $\mathbf{v}_0$. 
To build $\mathbf{f}_{0} \in \mathbb{R}^{N_c \times h_0 \times w_0}$, The left image $\mathbf{I}_l$ passes through another three layers of $3\times3$ 2D convolutions, similarly to the beginning of the feature extraction, to fit the size of the feature map to $\mathbf{v}_0$.
The cost aggregation convolves and fuses $\mathbf{f}_{0}$ and $\mathbf{v}_0$ to produce the cost volume $\mathbf{v}_{end} \in \mathbb{R} ^ {d_0 \times h_0 \times w_0}$.
% The cost aggregation module has two parallel paths of UNet structures to evolve each of the left feature map $\mathbf{f}_{0}$ and the cost volume $\mathbf{v}_0$. 
At each level of encoder and decoder, the 3D UNet for $\mathbf{v}_i$ has an input connection from the corresponding level of the 2D UNet evolving $\mathbf{f}_i$ as
\begin{align}
\begin{split}\label{eq:fenc}
    \mathbf{f}^\mathrm{Enc}_{i} = \operatorname{Enc}^{2d}\left(\mathbf{f}^\mathrm{Enc}_{i-1}\right)
\end{split}\\
\begin{split}\label{eq:fdec}
    \mathbf{f}^{\mathrm{Dec}}_{i} = \operatorname{Dec}^{2d}\left(\mathbf{f}^{\mathrm{Dec}}_{i+1}, \mathbf{f}^\mathrm{Enc}_{i}\right)
\end{split}\\
\begin{split}\label{eq:venc}
    \mathbf{v}^\mathrm{Enc}_{i} = \operatorname{Enc}^{3d}\left(\mathbf{v}^\mathrm{Enc}_{i-1}, \mathbf{f}^\mathrm{Enc}_{i}\right)
\end{split}\\
\begin{split}\label{eq:vdec}
    \mathbf{v}^{\mathrm{Dec}}_{i} = \operatorname{Dec}^{2d}\left(\mathbf{v}^{\mathrm{Dec}}_{i+1}, \mathbf{v}^\mathrm{Enc}_{i}, \mathbf{f}^\mathrm{Dec}_{i}\right)
\end{split}
\end{align}
where $\mathbf{f}^\mathrm{Enc}_{0} = \mathbf{f}_{0}$ and $\mathbf{v}^\mathrm{Enc}_{0} = \mathbf{v}_0$.
More details of cost aggregation will be described in the following subsections.

To recover the original resolution of the input images, the cost volume $\mathbf{v}^{\mathrm{Dec}}_{0}$ is up-sampled into the cost volume $\mathbf{V} \in \mathbb{R} ^ {D \times H \times W}$ by tri-linear interpolation. 
For each pixel, the disparity $\mathbf{d}$ is estimated with the soft argmax function\cite{kendall2017end},
\begin{align}
    \mathbf{d}\left(i, j\right)=\sum_{d=0}^{D-1} \frac{ e^{V(d,i,j)}}{\sum_{k} e^{V(k,i,j)}} d .
\end{align}

During all trainings, we use smooth L1 loss function $\mathcal{L}=\operatorname{smooth}_{L_1}\left(\mathbf{d} -\mathbf{d}_{\mathrm{gt}}\right)$, where
\begin{align}
    \operatorname{smooth}_{L_1}(x)=\left\{\begin{array}{lc}
    0.5 x^2, & |x|<1 \\
    |x|-0.5, & \text { otherwise }
    \end{array}\right.
\end{align}
with an end-to-end manner.


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{2D feature map and 3D volume fusion}
% Most of recent deep learning methods for stereo matching focuses on evolving the initialized cost volume built by matching the left and right feature maps to smooth and filter out the disparity surfaces.
% relies on geometric context in the 3D space.
% However, left image is kinds of 
The most straightforward way to merge the 2D feature map and 3D volume is to concatenate the 2D feature map at each sliced plane of the 3D volume along the disparity dimension.
However, in the appendix, we prove that the broadcasting sum of the feature map and the cost volume, each of which is processed by a 2D and 3D convolution, is equivalent to a 3D convolution on the concatenated cost volume but more efficient on computation and memory consumption.
Therefore, we apply the broadcasting sum between the feature maps $f_i$ and the cost volumes $v_i$ throughout the whole network structure.
% which is different with recent deep learning methods incorporating pipelines the left image at the last refinement.

In addition to broadcasting sum, we adopt atrous convolutions\cite{florian2017rethinking} on both 2D and 3D convolutions to involve larger receptive fields.
Each atrous block is the concatenation of three convolutions with different dilation as
\begin{align}
\begin{split}
& \footnotesize\text{As}^{2d}\left(x\right) =  \left\{{\footnotesize\text{Conv}}^{2d}_{_{|1,1|}}\left(x\right), {\footnotesize\text{Conv}}^{2d}_{_{|2,2|}}\left(x\right), {\footnotesize\text{Conv}}^{2d}_{_{|3,3|}}\left(x\right)\right\}
\end{split}\\
\begin{split}
& \footnotesize\text{As}^{3d}\left(x\right) =  \left\{{\footnotesize\text{Conv}}^{3d}_{_{|1,1,1|}}\left(x\right), {\footnotesize\text{Conv}}^{3d}_{_{|1,2,2|}}\left(x\right), {\footnotesize\text{Conv}}^{3d}_{_{|1,3,3|}}\left(x\right)\right\}
\end{split}
\end{align}
where ${\footnotesize\text{Conv}}^{Xd}_{_{|d|}}$ is X dimensional convolution with the kernel size 3, stride 1, and dilation $d$.
Both together...


The following subsection will describe the detailed usage of the broadcasting sum and the atrous block.


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{Image-coupled Volume Propagation}
\begin{figure*}[t]
  \begin{center}
  \includegraphics[width=1\linewidth]{imgs/model_abstract.png}
\end{center}
\caption{
The whole structure of the model. Our model evolves  
}
\label{fig:model}
\end{figure*}

For the following formulation, we denote the sequential operation of convolution, batch normalization\cite{ioffe2015batch}, and Leaky ReLU\cite{maas2013rectifier} as
\begin{align}
    \Phi^{Xd}_{k,s}\left(x\right) = \text{LeakyReLU}_{0.1}\left(\text{BN}\left({\footnotesize\text{Conv}}^{Xd}_{k,s}\left(x\right)\right)\right)
\end{align}
where ${\footnotesize\text{Conv}}^{Xd}_{k,s}$ is X-dimensional convolution with kernel size $k$ and stride $s$. We notate $s=2\uparrow$ for convolution with stride 2 to downsample and $s=2\downarrow$ for deconvolution with stride 2 to upsample the feature map or volume.


The 2D UNet pipeline has a structure similar to the original UNet, which consists of encoder layers to downsample the feature maps, and decoder layers to recover the resolutions and integrate the skip connections from the encoders as
\begin{align}
\begin{split}
    & \operatorname{Enc}^{2d} \left(\mathbf{f}^\mathrm{Enc}_{i-1}\right) = \Phi^{2d}_{3, 1}\left(\Phi^{2d}_{3,1}\left(\Phi^{2d}_{3,2\downarrow}\left(\mathbf{f}^\mathrm{Enc}_{i-1}\right)\right)\right)
\end{split}\\
\begin{split}
     \operatorname{Dec}^{2d} \left(\mathbf{f}^{\mathrm{Dec}}_{i+1}, \mathbf{f}^\mathrm{Enc}_{i}\right) 
    = \Phi^{2d}_{3,1}\left( \Phi^{2d}_{3,1}\left( \footnotesize\text{Skip}^{2d} \left(\mathbf{f}^{\mathrm{Dec}}_{i+1}, \mathbf{f}^\mathrm{Enc}_{i}\right)\right)\right)
\end{split}
\end{align}
where
\begin{align}
\begin{split}
    \footnotesize\text{Skip}^{Xd} \left(x^{\mathrm{Dec}}_{i+1}, x^\mathrm{Enc}_{i}\right) = \Phi^{Xd}_{1,1}\left(\Phi^{Xd}_{3,2\uparrow}\left(x^{\mathrm{Dec}}_{i+1}\right) \oplus x^\mathrm{Enc}_{i}\right)
\end{split}
\end{align}
and $\oplus$ is concatenation along the feature axis.
By concatenating the skip connection from the encoder part, the decoder layers keep detailed features on the upper resolutions while handling semantic information coming from lower resolutions.

While keeping similar encoder and decoder structures with skip connections to evolve the 3D volume $v_i$, the 3D UNet pipeline also has the connection from the 2D feature maps $f_i$.
The 2D-3D fusion is operated by broadcasting sum after the atrous blocks as
\begin{align}
\begin{split}
    &\operatorname{Enc} ^{3d}\left(\mathbf{v}^\mathrm{Enc}_{i-1}, \mathbf{f}^\mathrm{Enc}_{i}\right) \\
    & = \Phi^{3d}_{3,1}\left(\Phi^{3d}_{3,1}\left(\Psi\left(A\left(\Phi^{3d}_{3,2\downarrow}\left(\mathbf{v}^\mathrm{Enc}_{i-1}\right)\right) + B\left(\mathbf{f}^\mathrm{Enc}_{i}\right)\right)\right)\right)
\end{split} \\
\begin{split}
    &\operatorname{Dec}^{3d}\left(\mathbf{v}^{\mathrm{Dec}}_{i+1}, \mathbf{v}^\mathrm{Enc}_{i}, \mathbf{f}^\mathrm{Dec}_{i}\right) \\ &= \Phi^{3d}_{3,1}\left(\Psi\left(A\left(\footnotesize\text{Skip}^{3d} \left(\mathbf{v}^{\mathrm{Dec}}_{i+1}, \mathbf{v}^\mathrm{Enc}_{i} \right)\right)   +B\left(\mathbf{f}^\mathrm{Dec}_{i}\right)\right)\right)
\end{split}
\end{align}
where
\begin{align}
\begin{split}
    & A \left(\mathbf{v}^\mathrm{Enc}_{i}\right) 
     ={\footnotesize\text{Conv}}^{3d}_{1,1}\left(\Psi\left(\footnotesize\text{As}^{3d}\left(\mathbf{v}^\mathrm{Enc}_{i}\right)\right)\right)
\end{split} \\
\begin{split}
    & B\left(\mathbf{f}^\mathrm{Enc}_{i}\right)= 
    {\footnotesize\text{Conv}}^{2d}_{1,1}\left(\Psi\left(\footnotesize\text{As}^{2d}\left(\mathbf{f}^\mathrm{Enc}_{i}\right)\right)\right)
\end{split} \\
\begin{split}
    \Psi\left(x\right)=\text{LeakyReLU}_{0.1}\left(\text{BN}\left(x\right)\right).
\end{split}
\end{align}
To save GPU memory and computation, the last layer of $\operatorname{Dec}^{3d}$ exceptionally excludes the atrous block as
\begin{align}
\begin{split}
    & \mathbf{v}^\mathrm{Dec}_{0} = \\ & {\footnotesize\text{Conv}}^{3d}_{3,1}\left(\Psi\left(\Phi^{3d}_{3,1}\left(\Phi^{3d}_{3,2\uparrow}\left(\mathbf{v}^{\mathrm{Dec}}_{1}\right) \oplus \mathbf{v}^\mathrm{Enc}_{0}\right)
     +{\footnotesize\text{Conv}}^{2d}_{3,1}\left(\mathbf{f}^\mathrm{Dec}_{0}\right)\right)\right).
\end{split}
\end{align}




\begin{figure}[t]
  \begin{center}
  \includegraphics[width=1\linewidth]{imgs/fusion_2d_3d.png}
\end{center}
\caption{
Illustration of 2D-3D fusion by broadcasting sum. The broadcasting sum results in the same output as the 2D-3D feature concatenation while being more efficient on computation and memory consumption.
}
\label{fig:fusion}
\end{figure}


==> _03_backup2.tex <==
\section{Methods}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{Overview}
The proposed model has four steps: feature extraction, cost volume construction, cost aggregation, and disparity regression.
Given a pair of left and right images $\mathbf{I}_l, \mathbf{I}_l \in \mathbb{R} ^ {3 \times H \times W}$, the feature extractor, a UNet-like CNNs\cite{ronneberger2015u}, produces the feature maps $\mathrm{f}_l, \mathrm{f}_r \in \mathbb{R}^{c_f \times h_0 \times w_0}$ where $h_0 = \left \lfloor H / 3 \right \rfloor$ and $w_0 = \left \lfloor W / 3 \right \rfloor$. The feature extractor begins with three layers of $3\times3$ 2D convolutions with output channels of 16, 32, and 32 and strides of 1, 3, and 1 to scale down the images at the third resolution, followed by a 3-level UNet.
Since the initial cost volume is constructed by group-wise correlation\cite{guo2019group} that requires a high dimension of feature maps, we use an asymmetric encoder-decoder structure to increase the output channels of the feature extractor.
The numbers of channels are 32, 64, and 128 for each level of encoder layers and 128 for all decoder layers by keeping the numbers subtracted by the feature number from the skip connection at the deconvolution layers, $\eg$ the last deconvolution convolves 128-channels into 96-channels to concatenate 32-channels skip connection.

To operate group-wise correlation, each feature map $\mathrm{f} \in \mathbb{R}^{c_f \times h_0 \times w_0}$ is split along the channel dimension into $c_0$ number of feature maps $\left\{ \mathrm{f}^{1}, \mathrm{f}^{2}, ..., \mathrm{f}^{c_0}\right\}$ where each $\mathrm{f}^{g}$ has $c_f/c_0$ number of channels. 
Each value in the initial cost volume $\mathbf{v}_0 \in \mathbb{R} ^ {c_0 \times d_0 \times h_0 \times w_0}$ is determined as 
\begin{align}
    \mathbf{v}_0\left(g, d, i, j\right)=\frac{1}{c_f / c_0}\left\langle\mathrm{f}_l^g(i, j), \mathrm{f}_r^g(i, j-d)\right\rangle
\end{align}
where $d_0 = \left \lfloor D / 3 \right \rfloor$ and $D$ is the maximum disparity.

The cost aggregation module has two parallel paths of UNet structures to evolve another left feature map $\mathbf{f}_{0}$ as well as the 3D cost volume $\mathbf{v}_0$. 
To build $\mathbf{f}_{0} \in \mathbb{R}^{N_c \times h_0 \times w_0}$, The left image $\mathbf{I}_l$ passes through another three layers of $3\times3$ 2D convolutions, similarly to the beginning of the feature extraction, to fit the size of the feature map to $\mathbf{v}_0$.
The cost aggregation convolves and fuses $\mathbf{f}_{0}$ and $\mathbf{v}_0$ to produce the cost volume $\mathbf{v}_{end} \in \mathbb{R} ^ {d_0 \times h_0 \times w_0}$.
% The cost aggregation module has two parallel paths of UNet structures to evolve each of the left feature map $\mathbf{f}_{0}$ and the cost volume $\mathbf{v}_0$. 
At each level of encoder and decoder, the 3D UNet for $\mathbf{v}_i$ has an input connection from the corresponding level of the 2D UNet evolving $\mathbf{f}_i$ as
\begin{align}
\begin{split}\label{eq:fenc}
    \mathbf{f}^\mathrm{Enc}_{i} = \footnotesize\text{Enc}^{2d}\left(\mathbf{f}^\mathrm{Enc}_{i-1}\right)
\end{split}\\
\begin{split}\label{eq:fdec}
    \mathbf{f}^{\mathrm{Dec}}_{i} = \footnotesize\text{Dec}^{2d}\left(\mathbf{f}^{\mathrm{Dec}}_{i+1}, \mathbf{f}^\mathrm{Enc}_{i}\right)
\end{split}\\
\begin{split}\label{eq:venc}
    \mathbf{v}^\mathrm{Enc}_{i} = \footnotesize\text{Enc}^{3d}\left(\mathbf{v}^\mathrm{Enc}_{i-1}, \mathbf{f}^\mathrm{Enc}_{i}\right)
\end{split}\\
\begin{split}\label{eq:vdec}
    \mathbf{v}^{\mathrm{Dec}}_{i} = \footnotesize\text{Dec}^{2d}\left(\mathbf{v}^{\mathrm{Dec}}_{i+1}, \mathbf{v}^\mathrm{Enc}_{i}, \mathbf{f}^\mathrm{Dec}_{i}\right)
\end{split}
\end{align}
where $\mathbf{f}^\mathrm{Enc}_{0} = \mathbf{f}_{0}$ and $\mathbf{v}^\mathrm{Enc}_{0} = \mathbf{v}_0$.
Figure \ref{fig:model} shows the overall structure of the our cost aggregation module and more details will be described in the following subsections.

To recover the original resolution of the input images, the cost volume $\mathbf{v}^{\mathrm{Dec}}_{0}$ is up-sampled into the cost volume $\mathbf{V} \in \mathbb{R} ^ {D \times H \times W}$ by tri-linear interpolation. 
For each pixel, the disparity $\mathbf{d}$ is estimated with the soft argmax function\cite{kendall2017end},
\begin{align}
    \mathbf{d}\left(i, j\right)=\sum_{d=0}^{D-1} \frac{ e^{V(d,i,j)}}{\sum_{k} e^{V(k,i,j)}} d .
\end{align}

During all trainings, we use smooth L1 loss function $\mathcal{L}=\operatorname{smooth}_{L_1}\left(\mathbf{d} -\mathbf{d}_{\mathrm{gt}}\right)$, where
\begin{align}
    \operatorname{smooth}_{L_1}(x)=\left\{\begin{array}{lc}
    0.5 x^2, & |x|<1 \\
    |x|-0.5, & \text { otherwise }
    \end{array}\right.
\end{align}
with an end-to-end manner.


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{2D/3D fusion}
For the following formulations, we denote the sequential operation of convolution, batch normalization\cite{ioffe2015batch}, and Leaky ReLU\cite{maas2013rectifier} as
\begin{align}
    \Phi^{Xd}_{k,s}\left(x\right) = \footnotesize\text{LeakyReLU}_{0.1}\left(\footnotesize\text{BatchNorm}\left({\footnotesize\text{Conv}}^{Xd}_{k,s}\left(x\right)\right)\right)
\end{align}
where ${\footnotesize\text{Conv}}^{Xd}_{k,s}$ is X-dimensional convolution with kernel size $k$ and stride $s$. We notate $s=2\uparrow$ for convolution with stride 2 to downsample and $s=2\downarrow$ for deconvolution with stride 2 to upsample the feature map or volume.

% Most of recent deep learning methods for stereo matching focuses on evolving the initialized cost volume built by matching the left and right feature maps to smooth and filter out the disparity surfaces.
% relies on geometric context in the 3D space.
% However, left image is kinds of 
A straightforward way to merge the 2D feature map and 3D volume is to concatenate the 2D feature map at each sliced plane of the 3D volume along the disparity dimension.

A feature embeds geometric contexts on the 3D cost volume and image features. %%%%%%

A concatenated volume $v'$ can be formulated as
\begin{align}
\begin{split}
    \mathbf{v}'\left(c, d, i, j\right) = \left\{\begin{array}{lc}
    \mathbf{v}\left(c, d, i, j\right), & 1 \leq c \leq C_v \\
    \mathbf{f}\left(c - C_v, i, j\right), & C_v+1 \leq c \leq C_v + C_f
    \end{array}\right.
\end{split}
\end{align}
where $C_v$ and $C_f$ are the numbers of feature dension for $v$ and $f$.
\begin{align}
\begin{split}
    &\text{Conv}^{3d}_{k,s}\left(\mathbf{v}'; W_{v'} \right)\left(c, d, i, j\right)
\\ = &\sum_{\bar{c}} \sum_{\bar{d}} \sum_{\bar{i}} \sum_{\bar{j}} w_{\bar{c},\bar{d},\bar{i},\bar{j}}\mathbf{v}'\left(c+\bar{c}, d+\bar{d}, i+\bar{i}, j+\bar{j}\right) 
\\ = &\sum_{\bar{c}=1}^{C_v} \sum_{\bar{d}} \sum_{\bar{i}} \sum_{\bar{j}} w_{\bar{c},\bar{d},\bar{i},\bar{j}}\mathbf{v}\left(c+\bar{c}, d+\bar{d}, i+\bar{i}, j+\bar{j}\right) \\ &+ \sum_{\bar{c}=1}^{C_f} \sum_{\bar{d}} \sum_{\bar{i}} \sum_{\bar{j}} w_{\bar{c}+C_v,\bar{d},\bar{i},\bar{j}}\mathbf{f}\left(c - C_v +\bar{c}, i+\bar{i}, j+\bar{j}\right) 
\\ = &\sum_{\bar{c}=1}^{C_v} \sum_{\bar{d}} \sum_{\bar{i}} \sum_{\bar{j}} w_{\bar{c},\bar{d},\bar{i},\bar{j}}\mathbf{v}\left(c+\bar{c}, d+\bar{d}, i+\bar{i}, j+\bar{j}\right) \\ &+ \sum_{\bar{c}=1}^{C_f} \sum_{\bar{i}} \sum_{\bar{j}} \left(\sum_{\bar{d}} w_{\bar{c}+C_v,\bar{d},\bar{i},\bar{j}} \right)\mathbf{f}\left(c - C_v +\bar{c}, i+\bar{i}, j+\bar{j}\right) 
\\ = &\text{Conv}^{3d}_{k,s}\left(\mathbf{v}; W_v \right)\left(c, d, i, j\right)
+ \text{Conv}^{2d}_{k,s}\left(\mathbf{f}; W_f \right)\left(c, i, j\right)
\end{split}
\end{align}



\begin{figure}[t]
  \begin{center}
  \includegraphics[width=1\linewidth]{imgs/fusion_2d_3d.png}
\end{center}
\caption{
Illustration of 2D-3D fusion by broadcasting sum. The broadcasting sum results in the same output as the 2D-3D feature concatenation while being more efficient on computation and memory consumption.
}
\label{fig:fusion}
\end{figure}



However, in the appendix, we prove that the broadcasting sum of a feature map and a cost volume, each of which is processed by a 2D and 3D convolution, is equivalent to a 3D convolution on the concatenated cost volume but more efficient on computation and memory consumption.
Therefore, we apply the broadcasting sum between the feature maps $f_i$ and the cost volumes $v_i$ throughout the whole network structure.
% which is different with recent deep learning methods incorporating pipelines the left image at the last refinement.

In addition to broadcasting sum, we adopt atrous convolutions\cite{florian2017rethinking} on both 2D and 3D outputs to involve larger receptive fields.
Each atrous block is the concatenation of three convolutions with different dilations as
\begin{align}
\begin{split}
& \gamma^{2d}\left(x\right) =  \left\{{\footnotesize\text{Conv}}^{2d}_{_{|1,1|}}\left(x\right), {\footnotesize\text{Conv}}^{2d}_{_{|2,2|}}\left(x\right), {\footnotesize\text{Conv}}^{2d}_{_{|3,3|}}\left(x\right)\right\}
\end{split}\\
\begin{split}
& \gamma^{3d}\left(x\right) =  \left\{{\footnotesize\text{Conv}}^{3d}_{_{|1,1,1|}}\left(x\right), {\footnotesize\text{Conv}}^{3d}_{_{|1,2,2|}}\left(x\right), {\footnotesize\text{Conv}}^{3d}_{_{|1,3,3|}}\left(x\right)\right\}
\end{split}
\end{align}
where ${\footnotesize\text{Conv}}^{Xd}_{_{|d|}}$ is X dimensional convolution with the kernel size 3, stride 1, and dilation $d$.

All in all, the fusion module for a 2D feature map and a 3D volume is formulated as
\begin{align}
\begin{split}
    \mathcal{F}\left(\mathbf{v}, \mathbf{f}\right) = 
    \Phi^{3d}_{3,1}\left(\Psi\left(\Gamma^{3d}\left(\mathbf{v}\right) + \Gamma^{2d}\left(\mathbf{f}\right)\right)\right)
\end{split}
\end{align}
where $+$ is the boradcasting sum and
\begin{align}
\begin{split}
    \Gamma^{Xd}\left(x\right) = {\footnotesize\text{Conv}}^{Xd}_{1,1}\left(\Psi\left(\gamma^{Xd}\left(x\right)\right)\right)
    \\
\end{split}\\
\begin{split}
    \Psi\left(x\right)=\footnotesize\text{LeakyReLU}_{0.1}\left(\footnotesize\text{BatchNorm}\left(x\right)\right).
\end{split}
\end{align}
The following subsection will describe the detailed usage of the fusion blocks.


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\subsection{Image-coupled Volume Propagation}
\label{sec:methods}
\begin{figure*}[t]
  \begin{center}
  \includegraphics[width=1\linewidth]{imgs/model.png}
\end{center}
\caption{
The whole structure of the model. Our model consists of two paths for the 2D feature maps $\mathbf{f}_i$ and the 3D cost volume $\mathbf{v}_i$ each of which has UNet-like structures. Each output from a 2D block is connected to the corresponding 3D block with atrous convolution and broadcasting sum.
}
\label{fig:model}
\end{figure*}

The 2D pipeline has a similar structure to the original UNet, which consists of encoder layers to downsample the feature maps, and decoder layers to recover the resolutions and integrate the skip connections from the encoders as
\begin{align}
\begin{split}
    & \footnotesize\text{Enc}^{2d} \left(\mathbf{f}^\mathrm{Enc}_{i-1}\right) = \Phi^{2d}_{3, 1}\left(\Phi^{2d}_{3,1}\left(\Phi^{2d}_{3,2\downarrow}\left(\mathbf{f}^\mathrm{Enc}_{i-1}\right)\right)\right)
\end{split}\\
\begin{split}
     \footnotesize\text{Dec}^{2d} \left(\mathbf{f}^{\mathrm{Dec}}_{i+1}, \mathbf{f}^\mathrm{Enc}_{i}\right) 
    = \Phi^{2d}_{3,1}\left( \Phi^{2d}_{3,1}\left( \footnotesize\text{Skip}^{2d} \left(\mathbf{f}^{\mathrm{Dec}}_{i+1}, \mathbf{f}^\mathrm{Enc}_{i}\right)\right)\right)
\end{split}
\end{align}
where
\begin{align}
\begin{split}
    \footnotesize\text{Skip}^{Xd} \left(x^{\mathrm{Dec}}_{i+1}, x^\mathrm{Enc}_{i}\right) = \Phi^{Xd}_{1,1}\left(\Phi^{Xd}_{3,2\uparrow}\left(x^{\mathrm{Dec}}_{i+1}\right) \oplus x^\mathrm{Enc}_{i}\right)
\end{split}
\end{align}
and $\oplus$ is concatenation along the feature axis.
By concatenating the skip connection from the encoder part, the decoder layers are able to keep the detailed features on the upper resolutions while handling semantic information coming from lower resolutions.

While keeping similar encoder and decoder structures with the skip connections in order to evolve the 3D volume $v_i$, the 3D UNet pipeline also has the connection from the 2D feature maps $f_i$.
The 2D-3D fusion is operated by broadcasting sum after the atrous blocks as
\begin{align}
\begin{split}
    &\footnotesize\text{Enc} ^{3d}\left(\mathbf{v}^\mathrm{Enc}_{i-1}, \mathbf{f}^\mathrm{Enc}_{i}\right) = \Phi^{3d}_{3,1}\left(\mathcal{F}\left(\Phi^{2d}_{3,2\downarrow}\left(\mathbf{v}^\mathrm{Enc}_{i-1}\right), \mathbf{f}^\mathrm{Enc}_{i}\right)\right)
\end{split} \\
\begin{split}
    &\footnotesize\text{Dec}^{3d}\left(\mathbf{v}^{\mathrm{Dec}}_{i+1}, \mathbf{v}^\mathrm{Enc}_{i}, \mathbf{f}^\mathrm{Dec}_{i}\right) = 
    \mathcal{F}\left(\footnotesize\text{Skip}^{3d} \left(\mathbf{v}^{\mathrm{Dec}}_{i+1}, \mathbf{v}^\mathrm{Enc}_{i} \right), \mathbf{f}^\mathrm{Dec}_{i}\right)
\end{split}
\end{align}

Since the last layers of the cost volumes have the largest resolution which dominantly take GPU memory and computation power, we define a ligther $\footnotesize\text{Dec}^{3D}$ at the last layer without the atrous block as
\begin{align}
\begin{split}
    \mathbf{v}^\mathrm{Dec}_{0} =  {\footnotesize\text{Conv}}^{3d}_{3,1}\left(\Psi\left({\footnotesize\text{Conv}}^{3d}_{3,1}\left( \mathbf{v}^\mathrm{Dec}_{0, skip} \right)
     +{\footnotesize\text{Conv}}^{2d}_{3,1}\left(\mathbf{f}^\mathrm{Dec}_{0}\right)\right)\right)
\end{split}
\end{align}
where $\mathbf{v}^\mathrm{Dec}_{0, skip} = \Phi^{3d}_{3,2\uparrow}\left(\mathbf{v}^{\mathrm{Dec}}_{1}\right) \oplus \mathbf{v}^\mathrm{Enc}_{0}$.




==> imgs/mb.tex <==

% \begin{figure*}[t]
% \begin{subfigure}{0.33\linewidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{imgs/mb2_im0.png}
%   \caption{"Bicycle2" image}
% \end{subfigure}%
% \begin{subfigure}{0.33\linewidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{imgs/mb8_im0.png}
%   \caption{"Djembe" image}
% \end{subfigure}
% \begin{subfigure}{0.33\linewidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{imgs/mb3_im0.png}
%   \caption{"Classroom2" image}
% \end{subfigure} 
% \begin{subfigure}{0.33\linewidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{imgs/mb2_disp0.png}
%   \caption{"Bicycle2" result}
% \end{subfigure}
% \begin{subfigure}{0.33\linewidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{imgs/mb8_disp0.png}
%   \caption{"Djembe" result}
% \end{subfigure}
% \begin{subfigure}{0.33\linewidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{imgs/mb3_disp0.png}
%   \caption{"Classroom2" result}
% \end{subfigure}
% \caption{
% Qualitative comparison on Middlebury V3
% }
% \label{fig:mb}
% \end{figure*}






\begin{figure*}[t]
\begin{subfigure}{0.245\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{imgs/mb2_im0.png}
  \caption{"Bicycle2" image}
\end{subfigure}%
\begin{subfigure}{0.245\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{imgs/mb2_lea.jpg}
  \caption{LEAStereo\cite{cheng2020hierarchical}}
\end{subfigure}
\begin{subfigure}{0.245\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{imgs/mb2_hitnet.jpg}
  \caption{HITNet\cite{tankovich2021hitnet}}
\end{subfigure} 
\begin{subfigure}{0.245\linewidth}
  \centering
  \includegraphics[width=.99\linewidth]{imgs/mb2_ours.jpg}
  \caption{Ours}
\end{subfigure}
\label{fig:mb2}
\end{figure*}

